eSIM Technology in IoT Architecture

eSIM(embedded SIM) is an advanced alternative to traditional physical SIM cards initially developed by the GSM Association(GSMA) in 2013 [1][2]. The eSIM technology has been deployed in many commercial products such as mobile devices. However, the application of the eSIM technology in IoT devices has yet to start being primarily deployed. Understanding the eSIM architecture and the basic ideas of the eSIM provisioning and operations is very important for engineers to promote eSIM technology deployment in more areas, both academics and industries. The report focuses on the eSIM technology in the IoT architecture and two major operations of Remote SIM Provisioning(RSP) procedure: the Common Mutual Authentication procedure, a process used to authenticate eSIM trusted communication parties over the public internet, and the Profile Downloading procedure, the way to download the Profile from the operator SM-DP+ server and eventually remotely provision the end-user devices.

==> fig-cancel-common-mutual-authentication.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.5]{figures/fig-cancel-common-mutual-authentication.png}
    \caption{Cancel Common Mutual Authentication Procedure}
    \label{fig:cancel-common-mutual-authentication}
\end{figure}
